Predicting Individual Depression Symptoms from Acoustic Features During Speech

Current automatic depression detection systems provide predictions directly without relying on the individual symptoms/items of depression as denoted in the clinical depression rating scales. In contrast, clinicians assess each item in the depression rating scale in a clinical setting, thus implicitly providing a more detailed rationale for a depression diagnosis. In this work, we make a first step towards using the acoustic features of speech to predict individual items of the depression rating scale before obtaining the final depression prediction. For this, we use convolutional (CNN) and recurrent (long short-term memory (LSTM)) neural networks. We consider different approaches to learning the temporal context of speech. Further, we analyze two variants of voting schemes for individual item prediction and depression detection. We also include an animated visualization that shows an example of item prediction over time as the speech progresses.

==> tables/table_depression_detection_severity.tex <==
\begin{table}[!tbp]
\label{table:detection_severity_metrics}
\caption{Metrics for depression detection (F Score) and severity estimation (RSME). Models with 'I-' prefix indicate the Logistic/Linear regressions that were trained with the predictions from the models trained on individual depression items.}
\centering
\begin{tabular}{lcccc} 
\toprule
 Model & F  & F(ND) & F(D) & RMSE\\
\midrule
\multicolumn{5}{c}{\textbf{AASS}} \\ 
\midrule
Spec CNN& \multicolumn{1}{c}{0.7000} & \multicolumn{1}{c}{0.8000} & \multicolumn{1}{r}{0.5000} & \multicolumn{1}{c}{9.0142}  \\
Spec CNNLSTM & \multicolumn{1}{c}{0.7569} & \multicolumn{1}{c}{0.8276} & \multicolumn{1}{r}{0.6154} & \multicolumn{1}{c}{9.6055}  \\
eGeMAPS CNN & \multicolumn{1}{c}{0.8095} & \multicolumn{1}{c}{0.8571} & \multicolumn{1}{r}{0.7143} & \multicolumn{1}{c}{8.5475}  \\ 
\midrule
I-Spec CNN  & 0.7000 & 0.8000& 0.5000  & 10.0164 \\
I-Spec CNNLSTM & 0.6190 & 0.7143& 0.4286  & 10.2242 \\
I-eGeMAPS CNN  & 0.5667 & 0.7500& 0.2000  & 10.0582 \\ 
\midrule
\multicolumn{5}{c}{\textbf{DAICWOZ}}  \\ 
\midrule
Spec CNN& \multicolumn{1}{c}{0.7011} & \multicolumn{1}{c}{0.8478} & \multicolumn{1}{c}{0.3000} & \multicolumn{1}{c}{5.7466}  \\
Spec CNNLSTM & \multicolumn{1}{c}{0.6990} & \multicolumn{1}{c}{0.8140} & \multicolumn{1}{c}{0.3846} & \multicolumn{1}{c}{5.6559}  \\
eGeMAPS CNN & \multicolumn{1}{c}{0.7131} & \multicolumn{1}{c}{0.8276} & \multicolumn{1}{c}{0.4000} & \multicolumn{1}{c}{5.9478}  \\ 
\midrule
I-Spec CNN  & 0.7144 & 0.8602& 0.3158  & 6.2597  \\
I-Spec CNNLSTM & 0.6622 & 0.8090& 0.2609  & 6.0484  \\
I-eGeMAPS CNN  & 0.7411 & 0.8409& 0.4615  & 6.3786  \\\bottomrule
\end{tabular}
\end{table}

==> tables/table_multitask_AASS_sp1.tex <==
\begin{table*}[!htbp]
\caption{Comparison of the model performance (for each individual item of MADRS) obtained using multi-task and single-task models. Results are presented in terms of Weighted FScore. Results obtained using the AASS dataset
} 
\label{table:wfs_aass_multitask_sp}
\centering
\begin{tabular}{l|cccccccc} 
\toprule
& \multicolumn{4}{c}{\textbf{Hard Voting}} & \multicolumn{4}{c}{\textbf{Soft Voting}} \\
& \multicolumn{2}{c}{\textbf{Multi-task}} & \multicolumn{2}{c}{\textbf{Single-task}} & \multicolumn{2}{c}{\textbf{Multi-task}} & \multicolumn{2}{c}{\textbf{Single-task}} \\
\midrule
 \begin{tabular}[c]{@{}c@{}}Item - MADRS\\(AASS dataset) \end{tabular}& \begin{tabular}[c]{@{}c@{}}Spec\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Spec\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} \\ 
\midrule
(1) Apparent sadness & 0.52 & \textbf{0.69} & 0.36 & 0.61 & 0.52 & \textbf{0.69} & 0.36 & 0.61 \\
(2) Reported sadness & 0.59 & 0.62 & 0.62 & \textbf{0.71} & 0.59 & 0.62 & 0.62 & \textbf{0.71} \\
(3) Inner tension & 0.62 & 0.49 & \textbf{0.67} & 0.65 & 0.62 & 0.45 & 0.62 & 0.65 \\
(4) Reduced sleep & 0.67 & 0.62 & 0.67 & \textbf{0.76} & 0.67 & 0.62 & 0.67 & \textbf{0.76} \\
(5) Reduced appetite & 0.58 & 0.58 & 0.49 & \textbf{0.65} & 0.58 & 0.58 & 0.49 & \textbf{0.65} \\
(6) Conc. difficulties & 0.57 & 0.53 & 0.41 & \textbf{0.66} & 0.57 & 0.53 & 0.53 & \textbf{0.66} \\
(7) Lassitude & \textbf{0.52} & 0.44 & 0.33 & 0.42 & \textbf{0.52} & \textbf{0.44} & 0.33 & 0.42 \\
(8) Inability to feel & 0.48 & 0.57 & 0.67 & 0.52 & 0.48 & 0.51 & \textbf{0.79} & 0.58 \\
(9) Pessimistic thoughts & \textbf{0.76} & 0.71 & \textbf{0.76} & 0.62 & \textbf{0.76} & 0.71 & 0.67 & 0.62 \\
(10) Suicidal thoughts & 0.68 & 0.70 & 0.70 & \textbf{0.75} & 0.68 & 0.70 & 0.70 &\textbf{0.75} \\ 
\end{tabular}
\end{table*}

==> tables/table_multitask_DAIC_egemaps.tex <==
\begin{table*}[!htbp]
\caption{Comparison of the model performance (for each individual item of MADRS) obtained using multi-task and single-task models. Results are presented in terms of Weighted FScore. Results obtained using the AASS dataset
} 
\label{table:wfs_aass_multitask_sp}
\centering
\begin{tabular}{l|cccccccc} 
\toprule
& \multicolumn{4}{c}{\textbf{Hard Voting}} & \multicolumn{4}{c}{\textbf{Soft Voting}} \\
& \multicolumn{2}{c}{\textbf{Single-task}} & \multicolumn{2}{c}{\textbf{Multi-task}} & \multicolumn{2}{c}{\textbf{Single-task}} & \multicolumn{2}{c}{\textbf{Multi-task}} \\
\midrule
 \begin{tabular}[c]{@{}c@{}}Item - MADRS\\(AASS dataset) \end{tabular}& \begin{tabular}[c]{@{}c@{}}eGeM\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeM\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeM\\C-L\end{tabular} &
\begin{tabular}[c]{@{}c@{}}eGeM\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spec\\C-L\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeM\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeM\\C-L\end{tabular} \\ 
\midrule
(1) Apparent sadness & 0.66 & 0.76 & 0.70 & 0.75 & 0.76 & 0.62 & \textbf{0.77} & 0.66 \\
(2) Reported sadness & 0.61 & 0.71 & 0.71 & 0.76 & 0.61 & 0.69 & 0.71 & \textbf{0.81} \\
(3) Inner tension & 0.69 & 0.69 & 0.65 & \textbf{0.75} & 0.69 & 0.69 & 0.65 & 0.69 \\
(4) Reduced sleep & 0.74 & 0.75 & \textbf{0.86} & 0.82 & 0.74 & 0.71 & \textbf{0.86} & 0.76 \\
(5) Reduced appetite & 0.62 & 0.55 & \textbf{0.72} & 0.69 & 0.62 & 0.55 & \textbf{0.72} & 0.69 \\
(6) Conc. difficulties & 0.63 & 0.71 & 0.66 & 0.71 & 0.69 & 0.71 & 0.65 & \textbf{0.81} \\
(7) Lassitude & 0.57 & 0.67 & \textbf{0.71} & 0.57 & 0.51 & 0.53 & \textbf{0.71} & 0.58 \\
(8) Inability to feel & 0.80 & 0.65 & 0.80 & 0.80 & 0.75 & 0.70 & 0.80 & \textbf{0.86} \\
(9) Pessimistic thoughts & 0.81 & 0.81 & \textbf{0.86} & \textbf{0.86} & \textbf{0.86} & 0.81 & \textbf{0.86} & \textbf{0.86} \\
(10) Suicidal thoughts & 0.90 & 0.62 & \textbf{0.71} & 0.75 & \textbf{0.91} & 0.56 & \textbf{0.71} & 0.77 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table_wfscore.tex <==
\begin{table*}[!tbp]
\caption{Performance of the models trained on each of the individual items. Each cell contains metrics in the format: Weighted FScore / FScore (ND) / FScore (D). Last row corresponds to models trained for Depression Detection (total score $\geq$ 10).} 
\label{table:wfscore}
\centering
\begin{tabular}{c|ccc|ccc} 
\hline
 & \multicolumn{3}{c|}{\textbf{AASS}} & \multicolumn{3}{c}{\textbf{DAICWOZ}} \\
\hline
 \begin{tabular}[c]{@{}c@{}}Item\end{tabular}& \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular}\\ 
\hline
(1)& .58/.73/.33 & .65/.76/.46 & .71/.77/.63 & .54/.60/.49 & .52/.47/.56 & .57/.57/.57\\
(2)& .71/.67/.75 & .81/.82/.80 & .57/.61/.53 & .54/.52/.55 & .55/.47/.62 & .61/.51/.70\\
(3)& .67/.63/.70 & .66/.59/.72 & .81/.80/.82 & .55/.44/.63 & .58/.44/.68 & .55/.47/.62\\
(4)& .86/.87/.84 & .76/.76/.76 & .81/.83/.78 & .65/.21/.84 & .66/.46/.75 & .60/.22/.76\\
(5)& .66/.86/.00 & .69/.82/.25 & .63/.83/.00 & .55/.26/.72 & .62/.34/.77 & .54/.50/.57\\
(6)& .57/.57/.57 & .66/.72/.59 & .63/.76/.46 & .52/.51/.53 & .54/.44/.63 & .59/.50/.68\\
(7)& .54/.75/.20 & .56/.53/.61 & .65/.76/.46 & .61/.74/.44 & .55/.60/.49 & .59/.61/.57\\
(8)& .79/.87/.67 & .69/.80/.50 & .90/.92/.88 & .62/.83/.11 & .72/.86/.38 & .66/.79/.36\\
(9)& .67/.67/.67 & .71/.70/.73 & .86/.86/.86 &-- & -- & -- \\
(10) & .75/.86/.29 & .75/.86/.29 & .90/.94/.75 & -- & -- & -- \\
\hline
\begin{tabular}[c]{@{}c@{}}Dep.\\Det.\end{tabular} & .70/.80/.50 & .76/.83/.62 & .81/.86/.71 & .70/.85/.30 & .70/.81/.38 & .71/.83/.40 \\
\hline
\end{tabular}
\end{table*}

==> tables/table_wfscore_AASS.tex <==
\begin{table*}[!tbp]
\caption{Track level FScores of the models trained on each of the individual items when using hard. Each cell contains metrics in the format: Weighted FScore / FScore (ND) / FScore (D).
% Last row corresponds to models trained for Depression Detection (total score $\geq$ 10).
} 
\label{table:wfs_aass_hard}
\centering
\begin{tabular}{l|cccc} 
\hline
 \begin{tabular}[c]{@{}c@{}}Item\end{tabular}& \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN-LSTM\end{tabular} \\ 
\hline
(1) Apparent sadness & 0.36/0.32/0.43 & 0.61/0.71/0.43 & 0.66/0.74/0.53 & 0.76/0.81/0.67 \\
(2) Reported sadness & 0.62/0.60/0.64 & 0.71/0.73/0.70 & 0.61/0.67/0.56 & 0.71/0.75/0.67 \\
(3) Inner tension & 0.67/0.63/0.70 &0.65/0.53/0.74 &0.69/0.57/0.79 & 0.69/0.57/0.79 \\
(4) Reduced sleep & 0.67/0.67/0.67 & 0.76/0.76/0.76 & 0.74/0.83/0.62 & 0.75/0.81/0.67 \\
(5) Reduced appetite & 0.49/0.65/0.00 & 0.65/0.79/0.22 & 0.62/0.75/0.20 & 0.55/0.73/0.00 \\
(6) Conc. difficulties &0.41/0.27/0.59 &0.66/0.72/0.59& 0.63/0.76/0.46 &0.71/0.75/0.67 \\
(7) Lassitude &0.33/0.46/0.13 & 0.42/0.40/0.45 &0.57/0.67/0.40 &0.67/0.72/0.59 \\
(8)  Inability to feel & 0.67/0.72/0.59 &0.52/0.62/0.38 & 0.80/0.86/0.71 & 0.65/0.76/0.46 \\
(9) Pessimistic thoughts &0.76/0.78/0.74 &0.62/0.60/0.64 & 0.81/0.82/0.80 & 0.81/0.82/0.80 \\
(10)  Suicidal thoughts & 0.70/0.74/0.53 &0.75/0.86/0.29 & 0.90/0.94/0.75 &0.62/0.69/0.31  \\
% \hline
% \begin{tabular}[c]{@{}c@{}}Dep.\\Det.\end{tabular} & .70/.80/.50 & .76/.83/.62 & .81/.86/.71 & .70/.85/.30 \\
\hline
\end{tabular}
\end{table*}

==> tables/table_wfscore_AASS_soft.tex <==
\begin{table*}[!tbp]
\caption{Track level FScores of the models trained on each of the individual items when using soft voting. Each cell contains metrics in the format: Weighted FScore / FScore (ND) / FScore (D).
% Last row corresponds to models trained for Depression Detection (total score $\geq$ 10).
} 
\label{table:wfs_aass_soft}
\centering
\begin{tabular}{l|cccc} 
\hline
 \begin{tabular}[c]{@{}c@{}}Item\end{tabular}& \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN-LSTM\end{tabular} \\ 
\hline
(1) Apparent sadness & 0.36/0.32/0.43 & 0.61/0.71/0.43 & 0.76/0.81/0.67 &0.62/0.69/0.50 \\
(2) Reported sadness & 0.62/0.60/0.64 &0.71/0.73/0.70 & 0.61/0.67/0.56 & 0.69/0.77/0.63 \\
(3) Inner tension & 0.62/0.56/0.67 &0.65/0.53/0.74 &0.69/0.57/0.79 & 0.69/0.57/0.79 \\
(4) Reduced sleep & 0.67/0.67/0.67 &0.76/0.76/0.76 &0.74/0.83/0.62 & 0.71/0.77/0.63 \\
(5) Reduced appetite & 0.49/0.65/0.00 &0.65/0.79/0.22 & 0.62/0.75/0.20 &0.55/0.73/0.00 \\
(6) Conc. difficulties & 0.53/0.55/0.50 & 0.66/0.72/0.59 & 0.69/0.79/0.57 & 0.71/0.75/0.67 \\
(7) Lassitude &0.33/0.46/0.13 &0.42/0.40/0.45 &0.51/0.64/0.29 &0.53/0.55/0.50 \\
(8)  Inability to feel & 0.79/0.87/0.67 &0.58/0.73/0.33 & 0.75/0.83/0.62 &0.70/0.79/0.57 \\
(9) Pessimistic thoughts & 0.67/0.67/0.67 &0.62/0.60/0.64 & 0.86/0.86/0.86 & 0.81/0.82/0.80 \\
(10)  Suicidal thoughts & 0.70/0.74/0.53 &0.75/0.86/0.29 & 0.90/0.94/0.75 & 0.56/0.58/0.44  \\
% \hline
% \begin{tabular}[c]{@{}c@{}}Dep.\\Det.\end{tabular} & .70/.80/.50 & .76/.83/.62 & .81/.86/.71 & .70/.85/.30 \\
\hline
\end{tabular}
\end{table*}

==> tables/table_wfscore_DAIC_hard.tex <==
\begin{table*}[!tbp]
\caption{Performance of the models trained on each of the individual items  on DAIC-WOZ dataset when using hard voting. Each cell contains metrics in the format: Weighted FScore / FScore (ND) / FScore (D).
% Last row corresponds to models trained for Depression Detection (total score $\geq$ 10).
} 
\label{table:wfs_aass_soft}
\centering
\begin{tabular}{l|cccc} 
\toprule
 \begin{tabular}[c]{@{}c@{}}Item - PHQ-8 \\ (DAIC-WOZ dataset)\end{tabular}& \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN-LSTM\end{tabular} \\ 
\midrule
(1) Little interest & 0.51/0.54/0.49 & 0.44/0.47/0.41 & 0.54/0.60/0.49 & \textbf{0.59/0.60/0.58}   \\
(2) Feeling down &0.45/0.35/0.55 &0.47/0.38/0.55 & \textbf{0.61/0.51/0.70} &0.43/0.38/0.47 \\
(3) Trouble sleeping &0.49/0.27/0.64 &\textbf{0.55/0.47}/0.62 &0.45/0.22/0.62 &0.51/0.32/\textbf{0.65} \\
(4) Feeling tired &\textbf{0.64/0.34/0.77} &0.59/0.22/0.75 &0.56/0.09/0.76 &0.53/0.14/0.70 \\
(5) Poor appetite &\textbf{0.55}/0.26/\textbf{0.72} &0.46/0.39/0.49 &0.48/0.29/0.59 &0.54/\textbf{0.43}/0.61 \\
(6) Self-disappointment &0.44/0.18/0.66 &\textbf{0.54/0.44}/0.63 &0.46/0.40/0.52 & 0.42/0.13/\textbf{0.67} \\
(7) Conc. difficulties &0.52/0.57/0.45 &0.52/0.51/\textbf{0.53} &\textbf{0.60/0.69}/0.48 & 0.57/0.68/0.44\\
(8) Slow/Agitated &0.61/0.75/0.28 &\textbf{0.68/0.80/0.37} &0.66/0.79/0.36 &0.61/0.77/0.23 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table_wfscore_DAIC_soft.tex <==
\begin{table*}[!tbp]
\caption{Track level FScores of the models trained on each of the individual items when using soft voting. Each cell contains metrics in the format: Weighted FScore / FScore (ND) / FScore (D).
% Last row corresponds to models trained for Depression Detection (total score $\geq$ 10).
} 
\label{table:wfs_aass_soft}
\centering
\begin{tabular}{l|cccc} 
\hline
 \begin{tabular}[c]{@{}c@{}}Item (PHQ-8)\end{tabular}& \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spectrogram\\CNN-LSTM\end{tabular} & \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN\end{tabular} &
 \begin{tabular}[c]{@{}c@{}}eGeMAPS\\CNN-LSTM\end{tabular} \\ 
\hline
(1) Little interest & 0.53/0.55/0.52 & 0.55/0.38/0.69 & 0.53/0.63/0.44 &  0.59/0.61/0.57  \\
(2) Feeling down & 0.49/0.55/0.44 & 0.47/0.38/0.55 & 0.49/0.34/0.62 & 0.48/0.47/0.49  \\
(3)  Trouble sleeping & 0.55/0.44/0.63 & 0.55/0.47/0.62 & 0.51/0.37/0.61 & 0.50/0.31/0.63 \\
(4) Feeling tired &0.64/0.34/0.77 &0.59/0.22/0.75 &0.56/0.09/0.76 &0.58/0.10/0.79 \\
(5) Poor apetite & 0.51/0.14/0.71 & 0.46/0.39/0.49 & 0.46/0.25/0.58 & 0.47/0.42/0.50 \\
(6) Self-disappointment &0.44/0.18/0.66 &0.50/0.44/0.55 &0.46/0.40/0.52 & 0.42/0.13/0.67 \\
(7) Conc. difficulties &0.59/0.61/0.57 &0.52/0.51/0.53 &0.55/0.60/0.49 &0.55/0.67/0.40 \\
(8) Slow/Agitated &0.60/0.77/0.17 &0.68/0.80/0.37 &0.64/0.78/0.30 &0.60/0.75/0.22 \\
\hline
\end{tabular}
\end{table*}
